SMILE: Infusing Spatial and Motion Semantics in Masked Video Learning

Masked video modeling, such as VideoMAE, is an effective paradigm for video self-supervised learning (SSL). However, they are primarily based on reconstructing pixel-level details on natural videos which have substantial temporal redundancy, limiting their capability for semantic representation and sufficient encoding of motion dynamics. To address these issues, this paper introduces a novel SSL approach for video representation learning, dubbed as SMILE, by infusing both spatial and motion semantics. In SMILE, we leverage image-language pretrained models, such as CLIP, to guide the learning process with their high-level spatial semantics. We enhance the representation of motion by introducing synthetic motion patterns in the training data, allowing the model to capture more complex and dynamic content. Furthermore, using SMILE, we establish a new self-supervised video learning paradigm capable of learning strong video representations without requiring any natural video data. We have carried out extensive experiments on 7 datasets with various downstream scenarios. SMILE surpasses current state-of-the-art SSL methods, showcasing its effectiveness in learning more discriminative and generalizable video representations. Code is available: https://github.com/fmthoker/SMILE

==> preamble.tex <==
%
% --- inline annotations
%
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{booktabs}
% \usepackage{subfig}
\usepackage{bbm}
\usepackage{times}
\usepackage{epsfig}
\usepackage{tabu}
\usepackage{multirow}
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{xpunctuate}
\usepackage{pifont}% http://ctan.org/pkg/pifont
\usepackage{color,colortbl}
% \usepackage[rgb,dvipsnames]{xcolor}
\usepackage{tabulary,overpic}
\usepackage{booktabs}       % professional-quality tables
\usepackage[normalem]{ulem}

\usepackage{amsmath}
\usepackage{cite}

\usepackage{scalerel}
\usepackage[accsupp]{axessibility}

%%%% Customized Packages %%%%
\usepackage{xcolor}
\usepackage{enumitem}
\usepackage{arydshln} % dashed hline
\usepackage{xspace}
\usepackage{booktabs}
\usepackage{colortbl}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{lipsum} % Just for generating dummy text, can be removed
\usepackage{gensymb} % for \degree

\usepackage{tabularx}

% Include other packages here, before hyperref.
\newcommand{\reals}[1]{\mathbb{R}^{#1}}
\newcommand{\set}[1]{\left\{{#1}\right\}}
\newcommand{\transpose}[1]{#1^\top}
\newcommand*\rot{\rotatebox{90}}

\newcommand{\seqset}{\mathcal{S}}
\newcommand{\enorm}[1]{\left\|{#1}\right\|_2}
\newcommand{\binary}[1]{\mathbb{B}^{#1}}
\newcommand{\one}{\mathbf{1}}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

% Customized colors
\definecolor{fyxcolor}{RGB}{0,128,255}
\definecolor{demphcolor}{RGB}{100,100,100}
\definecolor{citecolor}{RGB}{0,0,192} % \definecolor{citecolor}{RGB}{34,139,34}
\definecolor{GrayBG}{gray}{0.95}

\newenvironment{smalltable}[1]{ \footnotesize \begin{tabular}{#1} }{ \end{tabular} }

\def\x{$\times$}
\newcommand{\demph}[1]{\textcolor{demphcolor}{#1}}
\newcommand{\app}{\raise.17ex\hbox{$\scriptstyle\sim$}}
\newlength\savewidth\newcommand\shline{\noalign{\global\savewidth\arrayrulewidth
  \global\arrayrulewidth 1pt}\hline\noalign{\global\arrayrulewidth\savewidth}}
\newcommand{\tablestyle}[2]{\setlength{\tabcolsep}{#1}\renewcommand{\arraystretch}{#2}\centering\footnotesize}

%%%% Reference Commands %%%%
\newcommand{\Tref}[1]{Table~\ref{#1}}
\newcommand{\eref}[1]{Eq.~\eqref{#1}}
\newcommand{\Eref}[1]{Equation~\eqref{#1}}
\newcommand{\fref}[1]{Fig.~\ref{#1}}
\newcommand{\Fref}[1]{Figure~\ref{#1}}
\newcommand{\sref}[1]{Sec.~\ref{#1}}
\newcommand{\Sref}[1]{Section~\ref{#1}}
\newrobustcmd{\B}{\bfseries}

%%%% Tricks for Compact Layout %%%%
% Caption configuration 
\usepackage[labelsep=period]{caption}
\captionsetup{font=small}
\captionsetup[table]{aboveskip=3pt}
\captionsetup[table]{belowskip=2pt}
\captionsetup[figure]{aboveskip=5pt}
\captionsetup[figure]{belowskip=0pt}

% Reduce the margin before paragraph
\renewcommand{\paragraph}[1]{\vspace{0.2em}\noindent \textbf{#1 \hspace{0.2em}}}
\definecolor{lightcyan}{rgb}{0.88, 1.0, 1.0}

%%%% Macors %%%%

% Author comments
\newcommand{\gy}[1]{\textcolor{magenta}{{[GY: #1]}}}
\newcommand{\todo}[1]{\textcolor{MyDarkRed}{{[TODO: #1]}}}
\newcommand{\ya}[1]{\textcolor{blue}{{[yuki: #1]}}}

% Just for tutorial
\definecolor{MyDarkRed}{rgb}{0.66, 0.16, 0.16}
\definecolor{MyDarkBlue}{rgb}{0.16, 0.16, 0.66}
\newcommand{\dummycolor}{lightgray} 
\newcommand{\correct}[1]{\textcolor{MyDarkBlue}{#1 \checkmark}}
\newcommand{\wrong}[1]{\textcolor{MyDarkRed}{#1 $\times$}}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}

% Variable abbreviations
\newcommand{\MethodName}{AGreatDeepNet\xspace}

% Math notations
\newcommand{\energy}{E}
\newcommand{\mass}{m}
\newcommand{\speedoflight}{c}

%%%%%%%%%%%%%%%%%% Customized packages and settings (end) %%%%%%%%%%%%%%%%%%

\newcommand{\str}[1]{\textcolor{red}{{[STR: #1]}}}
\newcommand{\cs}[1]{\textcolor{magenta}{CS: #1}}
\newcommand{\md}[1]{\textcolor{green}{MD: #1}}
\newcommand{\mr}[1]{\textcolor{red}{MR: #1}}
\newcommand{\fm}[1]{\textcolor{blue}{FM: #1}}
\newcommand{\ours}{\textsc{sigma} }
%\textsc{sigma} 
